BUSTER: a "BUSiness Transaction Entity Recognition" dataset

Albeit Natural Language Processing has seen major breakthroughs in the last few years, transferring such advances into real-world business cases can be challenging. One of the reasons resides in the displacement between popular benchmarks and actual data. Lack of supervision, unbalanced classes, noisy data and long documents often affect real problems in vertical domains such as finance, law and health. To support industry-oriented research, we present BUSTER, a BUSiness Transaction Entity Recognition dataset. The dataset consists of 3779 manually annotated documents on financial transactions. We establish several baselines exploiting both general-purpose and domain-specific language models. The best performing model is also used to automatically annotate 6196 documents, which we release as an additional silver corpus to BUSTER.

==> tables/5-fold_cross_validation_v2.tex <==
\begin{table*}[ht!]
\centering
\small
\begin{tabular}{r|ccc}
    \toprule
    {} &  \multicolumn{3}{}{Folds} \\
    {} & {Training} & {Validation} & {Test}\\ 
    \midrule
        Run$_1$ & 1, 2, 3 & 4  & 5\\
        Run$_2$ & 5, 1, 2 & 3  & 4\\
        Run$_3$ & 4, 5, 1 & 2  & 3\\
        Run$_4$ & 3, 4, 5 & 1  & 2\\
        Run$_5$ & 2, 3, 4 & 5  & 1\\
    \bottomrule
    \end{tabular}\caption{The five permutations of folds used for 5-fold cross validation}\label{tab:5_fold_cross_validation}
\end{table*}

==> tables/annoations_evaluations_v1.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
%
% The outputs of annotation procedure v1
%
\begin{table*}[!htp]
\centering
\scriptsize
\begin{tabular}{rccccccc}
    \toprule
    \textbf{Family}     & \textbf{LABEL} & $\AgrSym{1}{2}$ & {$\MutAgrSymA{1}{2}$} & {$\MutAgrSymA{2}{1}$}  & $\CovSym{1}{2}$ & $\CovSym{2}{1}$   & $\kappa$ \\
    \midrule
    \Parties            & \BUYNGCOMPANY              & 0.6675 & 0.7653 & 0.8393 & 0.8722 & 0.7953 & 0.6967 \\
    \Parties            & \SELLINGCOMPANY}             & 0.5086 & 0.6520 & 0.6980 & 0.7800 & 0.7286 & 0.6439 \\
    \textbf{\Parties.\ACQUIREDCOMPANY}            & 0.5979 & 0.7143 & 0.7859 & 0.8371 & 0.7608 & 0.6537 \\
    \textbf{\Info.\ANNUALREVENUES}             & 0.5727 & 0.7590 & 0.7000 & 0.7545 & 0.8182 & 0.7205 \\
    \textbf{\Advisors.\CONSULTANT}                    & 0.7391 & 0.8947 & 0.8095 & 0.8261 & 0.9130 & 0.8490 \\
    \textbf{\Advisors.\GENERICCONSULTINGCOMPANY}  & 0.6990 & 0.7697 & 0.8839 & 0.9082 & 0.7908 & 0.8128 \\
    \textbf{\Advisors.\LEGALCONSULTINGCOMPANY}    & 0.8839 & 0.9000 & 0.9802 & 0.9821 & 0.9018 & 0.9362 \\
    %\textbf{\Info.LOI\_DATE}                & 0.0571 & 0.0571 & 1.0000 & 1.0000 & 0.0571 & 0.1070 \\
    \midrule
    \textbf{MICRO OVERALL}                          & 0.6266 & 0.7343 & 0.8103 & 0.8533 & 0.7733 & 0.7439 \\
    \textbf{MACRO OVERALL}                          & 0.5907 & 0.6890 & 0.8371 & 0.8700 & 0.7207 & 0.6775 \\
    \bottomrule
\end{tabular}
\caption{The internal annotation results reported by the two annotators.}
\label{table:buster_internal_assessment}
\end{table*}

==> tables/annotation_evaluations_v2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
%
% The outputs of annotation procedure v2
%
\begin{table*}[!h]
\centering
\tiny
\begin{tabular}{lrccccccc}
    \toprule
    \textbf{Data Point Family} & \textbf{Data Point} & $\AgrSym{1}{2}$ & $\CovSymT{1}{2}{1}$ & $\CovSymT{2}{1}{2}$ & $\MutAgrSymT{1}{2}{1}$ & $\MutAgrSymT{2}{1}{2}$ & $\CohenKSym$ \\
    \midrule
    \multirow{3}{*}{\Parties}
                        & \BUYINGCOMPANY                & 0.6514 & 0.8749 & 0.7764 & 0.7445 & 0.8389 & 0.6810 \\
                        & \SELLINGCOMPANY               & 0.5026 & 0.7900 & 0.7126 & 0.6362 & 0.7053 & 0.6383 \\
                        & \ACQUIREDCOMPANY              & 0.5611 & 0.8427 & 0.7184 & 0.6658 & 0.7811 & 0.6119 \\
    \midrule
    \multirow{3}{*}{\Advisors}
                        % & \CONSULTANT                   & 0.6667 & 0.7500 & 0.9167 & 0.8889 & 0.7273 & 0.7988 \\
                        & \GENERICCONSULTINGCOMPANY     & 0.6624 & 0.9108 & 0.7516 & 0.7273 & 0.8814 & 0.7862 \\
                        & \LEGALCONSULTINGCOMPANY       & 0.8913 & 0.9891 & 0.9022 & 0.9011 & 0.9880 & 0.9405 \\
    \midrule
    \multirow{1}{*}{\Info}
                        & \ANNUALREVENUES               & 0.5781 & 0.7590 & 0.7000 & 0.6894 & 0.7817 & 0.7246 \\
    \toprule
                        & \textbf{MICRO OVERALL}        & 0.6100 & 0.8583 & 0.7517 & 0.7107 & 0.8115 & 0.7257 \\
                        & \textbf{MACRO OVERALL}        & 0.6448 & 0.8566 & 0.7882 & 0.7504 & 0.8148 & 0.7402 \\
    \bottomrule
\end{tabular}
\caption{The quality assessment results of the output of the annotation process.}
\label{tab:buster_internal_assessment}
\end{table*}

==> tables/baseline_results_v1.tex <==
\begin{table*}[ht]
\centering
\small
\begin{tabular}{r|ccc|ccc}
    \toprule
    \textbf{Model}          &  $\mu$-\textbf{Precision} &  $\mu$-\textbf{Recall} & $\mu$-\textbf{F1} & M-\textbf{Precision} & M-\textbf{Recall} & M-\textbf{F1}\\ 
    \midrule
        BERT & 59.7 & 68.9 & 64.0 & 56.8  &   68.2  & 61.8\\
        SEC-BERT       & 66.5 &  74.2 & 70.1 & 63.6  & 69.5 &    65.8\\
        RoBERTa        & \textbf{68.8} & 75.5  & \textbf{72.0} &  \textbf{71.3} & \textbf{80.3} & \textbf{75.4}\\
        Longformer     &  67.1 & \textbf{76.5} & 71.5 & 69.6 &    77.7 & 73.2\\
    \bottomrule
    \end{tabular}\caption{Micro ($\mu$-) and macro (M-) scores of the four baseline models.}\label{tab:baselines_micro-f1}
\end{table*}

==> tables/baseline_results_v2.tex <==
\begin{table*}[ht!]
\centering
\small
\begin{tabular}{r|ccc|ccc}
    \toprule
    \textbf{Model}  &  $\mu$-\textbf{Precision} &  $\mu$-\textbf{Recall} & $\mu$-\textbf{F1} & M-\textbf{Precision} & M-\textbf{Recall} & M-\textbf{F1}\\ 
    \midrule
        BERT        & 59.98 $\pm$ 1.18 & 68.34 $\pm$ 0.99 & 63.90 $\pm$ 1.12 & 51.12 $\pm$ 3.87 & 61.62 $\pm$ 2.66 & 55.26 $\pm$ 2.97\\
        SEC-BERT    & 69.76 $\pm$ 2.64 & 73.94 $\pm$ 2.94 & 71.68 $\pm$ 0.64 & 66.86 $\pm$ 3.89 & 71.84 $\pm$ 4.41 & 69.06 $\pm$ 3.86\\
        \textbf{RoBERTa}     & 69.00 $\pm$ 1.42 & \textbf{75.36 $\pm$ 1.30} & \textbf{72.02 $\pm$ 0.70} & \textbf{70.98 $\pm$ 2.17} & \textbf{75.08 $\pm$ 3.90} & \textbf{72.42 $\pm$ 1.87}\\
        Longformer  & 67.00 $\pm$ 1.99 & 73.28 $\pm$ 1.49 & 70.00 $\pm$ 1.07 & 66.42 $\pm$ 5.14 & 70.42 $\pm$ 1.49 & 67.74 $\pm$ 2.92\\
    \bottomrule
    \end{tabular}\caption{Micro ($\mu$-) and macro (M-) scores of the four baseline models evaluated using 5-Fold Cross Validation.}\label{tab:baselines_micro-f1}
\end{table*}

==> tables/baseline_results_v3.tex <==
\begin{table*}[ht!]
\centering
\small
\begin{tabular}{r|ccc|ccc}
    \toprule
    \textbf{Model}  &  $\mu$-\textbf{Precision} &  $\mu$-\textbf{Recall} & $\mu$-\textbf{F1} & M-\textbf{Precision} & M-\textbf{Recall} & M-\textbf{F1}\\ 
    \midrule
        BERT        & 59.98 $\pm$ 1.06 & 68.34 $\pm$ 0.89 & 63.90 $\pm$ 1.00 & 51.12 $\pm$ 3.46 & 61.62 $\pm$ 2.38 & 55.26 $\pm$ 2.66\\
        
        SEC-BERT    & 67.00 $\pm$ 1.78 & 73.28 $\pm$ 1.34 & 70.00 $\pm$ 0.95 & 66.42 $\pm$ 4.60 & 70.42 $\pm$ 1.33 & 67.74 $\pm$ 2.61\\
        
        \textbf{RoBERTa}     & 69.00 $\pm$ 1.27 & \textbf{75.36 $\pm$ 1.16} & \textbf{72.02 $\pm$ 0.63} & \textbf{70.98 $\pm$ 1.93} & \textbf{75.08 $\pm$ 3.49} & \textbf{72.42 $\pm$ 1.67}\\
        
        Longformer  & 69.76 $\pm$ 2.36 & 73.94 $\pm$ 2.63 & 71.68 $\pm$ 0.57 & 66.86 $\pm$ 3.48 & 71.84 $\pm$ 3.94 & 69.06 $\pm$ 3.46\\
    \bottomrule
    \end{tabular}\caption{Micro ($\mu$-) and macro (M-) scores of the four baseline models evaluated using 5-Fold Cross Validation.}\label{tab:baselines_micro-f1}
\end{table*}

==> tables/baseline_results_v4.tex <==
\begin{table*}[ht!]
\centering
\small
\begin{tabular}{r|ccc|ccc}
    \toprule
    \textbf{Model}  &  $\mu$-\textbf{Precision} &  $\mu$-\textbf{Recall} & $\mu$-\textbf{F1} & M-\textbf{Precision} & M-\textbf{Recall} & M-\textbf{F1}\\ 
    \midrule
        BERT        & 60.58 $\pm$ 1.18 & 67.90 $\pm$ 1.50 & 64.02 $\pm$ 0.83 & 51.96 $\pm$ 4.37 & 60.96 $\pm$ 5.66 & 55.16 $\pm$ 4.38\\
        
        SEC-BERT    & 67.42 $\pm$ 1.06 & 73.28 $\pm$ 1.50 & 70.24 $\pm$ 0.86 & 67.78 $\pm$ 3.86 & 72.26 $\pm$ 3.16 & 69.72 $\pm$ 3.25\\
        
        \textbf{RoBERTa}     & 69.56 $\pm$ 0.80 & \textbf{75.72 $\pm$ 0.95} & \textbf{72.54 $\pm$ 0.47} & \textbf{71.96 $\pm$ 1.62} & \textbf{78.42 $\pm$ 2.19} & \textbf{74.78 $\pm$ 1.57}\\
        
        Longformer  & 70.74 $\pm$ 1.85 & 73.60 $\pm$ 1.39 & 72.14 $\pm$ 1.04 & 71.90 $\pm$ 3.53 & 78.08 $\pm$ 2.73 & 74.44 $\pm$ 1.49\\
    \bottomrule
    \end{tabular}\caption{Micro ($\mu$-) and macro (M-) scores of the four baseline models evaluated using 5-Fold Cross Validation.}\label{tab:baselines_micro-f1}
\end{table*}

==> tables/folds_stats_v1.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
%
% The 5-Fold statistics v1
%
\begin{table*}[!h]
    \centering
    \scriptsize
    \begin{tabular}{lllllllllll}
        \toprule
        \textbf{Used as} &\textbf{Name} & \textbf{N. docs} & \textbf{N. Annotations} & {\BUYINGCOMPANY} & {\SELLINGCOMPANY} & {\ACQUIREDCOMPANY} & {\CONSULTANT} & {\LEGALCONSULTINGCOMPANY} & {\GENERICCONSULTINGCOMPANY} & {\ANNUALREVENUES} \\
        \midrule
        \multirow{4}{*}{Training}
                    & $fold_1$  & 753  & 4129  & 1735 & 460  & 1398 & 19 & 141 & 253 & 123\\
                    & $fold_2$  & 759  & 4280  & 1802 & 447  & 1474 & 18 & 132 & 266 & 141\\
                    & $fold_3$  & 758  & 4117  & 1722 & 456  & 1362 & 22 & 151 & 258 & 146\\
                    & Total     & 2270 & 12526 & 5259 & 1363 & 4234 & 59 & 424 & 777 & 410\\
        \midrule
        \multirow{1}{*}{Validation}
                    & $fold_4$  & 755  & 4112  & 1707 & 426  & 1398 & 15 & 145 & 246 & 143\\
        \midrule
        \multirow{1}{*}{Test}
                    & $fold_5$  & 754  & 4179  & 1718 & 439  & 1447 & 24 & 152 & 256 & 143\\
        \bottomrule
    \end{tabular}
    \captionsetup{justification=centering}
    \caption{Folds statistics}
    \label{tab:fold_stats}
\end{table*}

==> tables/folds_stats_v2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
%
% The 5-Fold statistics v2
%
\begin{table*}[!h]
    \setlength\tabcolsep{2pt}
    \centering
    \small
    \begin{tabular}{cr|ccc|c|c|c|cc}
        \toprule
        &                             & \multicolumn{3}{c}{\textbf{Training}} &            & \textbf{Validation} & \textbf{Test} & \textbf{Silver} &\\
        &                             & \fold{1}  & \fold{2}  & \fold{3}  & \textbf{Total}    & \fold{4}   & \fold{5} & & \\
        \midrule
        & \textbf{N. Tokens}          & 685K     &  680K      & 687K      & 2052K &  697K      & 688K & 5647K  & \\
        & \textbf{N. Docs}            & 753       & 759       & 758       & 2270  & 755        & 754  & 6196   & \\
        & \textbf{N. Annotations}     & 4130      & 4277      & 4117      & 12524 & 4112       & 4179 & 33272  & \\
        \midrule
        \multirow{4}{*}{\Parties}
        & \BUYINGCOMPANY              & 1735      & 1800      & 1722      &  5257 & 1707       & 1718 & 14558 & \\
        & \SELLINGCOMPANY             &  460      &  447      &  456      &  1363 & 426        & 439  & 4016  & \\
        & \ACQUIREDCOMPANY            & 1399      & 1473      & 1362      &  4234 & 1430       & 1447 & 9879  & \\
        & \textbf{Total}              & 3594      & 3720      & 3540      & 10854 & 3563       & 3604 & 28453 & \\
        \midrule
        \multirow{4}{*}{\Advisors}
        & \CONSULTANT                 &  19       &  18       &  22       &   59  &  15        & 24 & 159   & \\
        & \LEGALCONSULTINGCOMPANY     & 141       & 132       & 151       &  424  & 145        & 152 & 1176 & \\
        & \GENERICCONSULTINGCOMPANY   & 253       & 266       & 258       &  777  & 246        & 256 & 2210 & \\
        & \textbf{Total}              & 413       & 416       & 431       & 1260  & 406        & 432 & 3545 & \\
        \midrule
        \multirow{2}{*}{\Info} 
        & \ANNUALREVENUES             & 123       & 141       & 146       & 410   & 143        & 143 & 1274 & \\
        & \textbf{Total}              & 123       & 141       & 146       & 410   & 143        & 143 & 1274 & \\
        \bottomrule
    \end{tabular}
    \caption{The 5-Fold and silver statistics.}
    \label{tab:fold_stats}
\end{table*}

==> tables/tag_wise_v1.tex <==
\begin{table*}[!h]
    \centering
    \small
    \begin{tabular}{cr|ccc}
     \toprule
        & \textbf{} &\textbf{Precision} & \textbf{Recall} & \textbf{F1}\\ 
     \midrule
     \multirow{3}{*}{\Parties}
        & \BUYINGCOMPANY & 72.0 & 78.9 & 75.3\\
        & \SELLINGCOMPANY & 59.7 & 77.9 & 67.6\\
        & \ACQUIREDCOMPANY & 66.0 & 67.5 & 66.8\\
    \midrule
    \multirow{3}{*}{\Advisors}
        & \CONSULTANT & 76.9 & 83.3 & 80.0\\
        & \LEGALCONSULTINGCOMPANY & 85.7 & 90.8 & 88.2\\
        & \GENERICCONSULTINGCOMPANY & 70.5 & 80.5 & 75.2\\
    \midrule
    \multirow{1}{*}{\Info}
        & \ANNUALREVENUES & 68.0 & 83.2 & 74.8\\
    \bottomrule
    \end{tabular}
    \caption{Tag-wise precision recall and f1-score obtained with the RoBERTa baseline.}
    \label{tab:roberta_cls_report}
\end{table*}

==> tables/tag_wise_v2.tex <==
\begin{table*}[ht!]
    \centering
    \small
    \begin{tabular}{cr|ccc}
     \toprule
        & \textbf{} &\textbf{Precision} & \textbf{Recall} & \textbf{F1}\\ 
     \midrule
     \multirow{3}{*}{\Parties}
        & \BUYINGCOMPANY   & 73.34 $\pm$ 1.95 & 77.62 $\pm$ 1.17 & 75.40 $\pm$ 1.18\\
        & \SELLINGCOMPANY  & 63.64 $\pm$ 2.35 & 74.44 $\pm$ 3.15 & 68.52 $\pm$ 0.77\\
        & \ACQUIREDCOMPANY & 63.80 $\pm$ 1.39 & 71.08 $\pm$ 1.95 & 67.22 $\pm$ 0.70\\
    \midrule
    \multirow{3}{*}{\Advisors}
        & \CONSULTANT               & 72.36 $\pm$ 10.24 & 57.88 $\pm$ 17.30 & 62.48 $\pm$ 10.99\\
        & \LEGALCONSULTINGCOMPANY   & 83.52 $\pm$ 3.12  & 90.56 $\pm$ 1.22  & 86.88 $\pm$ 1.63\\
        & \GENERICCONSULTINGCOMPANY & 74.86 $\pm$ 2.34  & 77.86 $\pm$ 4.89  & 76.18 $\pm$ 2.02\\
    \midrule
    \multirow{1}{*}{\Info}
        & \ANNUALREVENUES & 65.5 $\pm$ 1.78 & 76.22 $\pm$ 7.29 & 70.23 $\pm$ 3.00\\
    \bottomrule
    \end{tabular}
    \caption{Tag-wise precision, recall and F1-score values obtained with\\ the RoBERTa baseline using 5-Fold Cross Validation.}
    \label{tab:roberta_cls_report}
\end{table*}

==> tables/tags_occurrence.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
%
% The 5-Fold statistics v2
%
\newcommand{\rg}[4]{\phantom{#1}#2-\phantom{#3}#4}
\begin{table*}[ht!]
    \centering
    \scriptsize
    \begin{tabularx}{\textwidth}{cr|ccc|c|c|c}
        \toprule
        &                             & \multicolumn{3}{c}{\textbf{Training}} &        & \textbf{Validation} & \textbf{Test}\\
        &                             & \fold{1}  & \fold{2}  & \fold{3}  & \textbf{Total}    & \fold{4}   & \fold{5}\\
        \midrule
        \multirow{4}{*}{\Parties}
        & \BUYINGCOMPANY              & \rg{00}{8}{}{1419}  & \rg{0}{10}{}{1462} & \rg{00}{8}{}{1514} & \rg{00}{8}{}{1514} & \rg{00}{8}{}{1411} & \rg{00}{8}{}{1391} \\
        & \SELLINGCOMPANY             & \rg{00}{8}{0}{943}  & \rg{0}{10}{}{1012} & \rg{0}{12}{}{1124} & \rg{00}{8}{}{1124} & \rg{0}{12}{}{1104} & \rg{0}{10}{}{1150} \\
        & \ACQUIREDCOMPANY            & \rg{0}{14}{}{1541}  & \rg{0}{14}{}{1467} & \rg{0}{11}{}{1342} & \rg{0}{11}{}{1541} & \rg{0}{13}{}{1375} & \rg{0}{13}{}{1481} \\
        & \textbf{Total}              & \rg{00}{8}{}{1541}  & \rg{0}{10}{}{1467} & \rg{0}{12}{}{1514} & \rg{00}{8}{}{1514} & \rg{00}{8}{}{1411} & \rg{00}{8}{}{1481} \\
        \midrule
        \multirow{4}{*}{\Advisors}
        & \CONSULTANT                 & \rg{}{138}{}{1156} & \rg{}{129}{}{1002} & \rg{0}{64}{}{1006} & \rg{0}{64}{}{1156} & \rg{}{113}{}{1542} & \rg{}{125}{}{1365} \\
        & \LEGALCONSULTINGCOMPANY     & \rg{}{182}{}{1325} & \rg{}{189}{}{1197} & \rg{}{218}{}{1332} & \rg{}{182}{}{1332} & \rg{}{160}{}{1732} & \rg{}{192}{0}{968} \\
        & \GENERICCONSULTINGCOMPANY   & \rg{0}{83}{}{1337} & \rg{0}{53}{}{1191} & \rg{0}{55}{}{1334} & \rg{0}{53}{}{1337} & \rg{0}{67}{}{1720} & \rg{}{103}{}{1032} \\
        & \textbf{Total}              & \rg{0}{83}{}{1337} & \rg{0}{53}{}{1197} & \rg{0}{55}{}{1334} & \rg{0}{53}{}{1337} & \rg{}{160}{}{1732} & \rg{}{125}{}{1365} \\
        \midrule
        \multirow{2}{*}{\Info} 
        & \ANNUALREVENUES             & \rg{0}{33}{}{1141} & \rg{0}{31}{}{1136} & \rg{0}{55}{}{1334} & \rg{0}{33}{}{1334} & \rg{0}{28}{}{1140} & \rg{0}{34}{}{1297} \\
        & \textbf{Total}              & \rg{0}{33}{}{1141} & \rg{0}{31}{}{1136} & \rg{0}{55}{}{1334} & \rg{0}{33}{}{1334} & \rg{0}{28}{}{1140} & \rg{0}{34}{}{1297} \\
        \bottomrule
    \end{tabularx}
    \caption{The token of the first--last occurrence of each tag and family of tags.}
    \label{tab:fold_tags_occurrences}
\end{table*}

==> tables/tagset_v1.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  The TAGSET Structure v1
%
\begin{comment}
\begin{itemize}
    \item[(a)] \Companies\\ 
    Set of labels used to identify the companies directly involved in the transaction.
    We decided to use this label only when the role of a company in the transaction is linguistically evident. 
    In addition, we also decided not to include the abbreviation in parentheses that often appears after the company name.\\
    \begin{itemize}
        \item \ACQUIREDCOMPANY\\
            This label is used to identify the company being acquired in the transaction. 
            However, in documents, the target entity in a transaction could also be a ``legal entity'', ``an asset'', a ``business division'', a ``real estate'' or ``mineral property''; in other words, it could be any revenue generating business or asset. 
            We decided to use this label only when the entity being purchased is a company or a part of its capital (for example a percentage of it), thus excluding cases of asset acquisition.\\
            
        \item \BUYINGCOMPANY\\
            The label is used to identify the company that acquires the target entity in a transaction.
            In this case, we decided to also include the cases in which the target entity is not a company and in which, therefore, the transaction also involve only assets.
            Moreover, the acquiring company may also refer to a person, a family, individual investors, a consortium, etc.
            In the case the document mentions a parent and a subsidiary company, and the latter is doing the acquisition, we consider the parent company as the buyer. 
            In the case of a merger, we assumed the first company mentioned as Buying Company and the second as Acquired Company.
            Finally, in the case of a joint venture, we decided to label the name of the joint venture, ignoring the individual parties involved in the business agreement.\\
            
        \item \SELLINGCOMPANY\\
            The label is used to identify the company selling the target entity in a transaction.
            Similarly to the case of the buying company, we have decided to consider a selling company even when the entity they are selling is not a company but an asset.\\
    \end{itemize}
    \item[(b)] \Advisors\\
    Set of labels defined to identify any external facilitators and advisors of the transaction.
    Similarly to the companies case, we decided to consider the entity only when occurring in contexts where a clear linguistic evidence that it is an advisor exists.\\
    \begin{itemize}
        \item \CONSULTANT\\
        Individual professionals (either independent or of respective consulting firm) advising on the transactions.\\
        
        \item \LEGALCONSULTINGCOMPANY\\
        A law firm providing advice on mergers and acquisitions, private equity matters, government regulation, litigation, anti-trust, structured finance, tax etc.\\
        
        \item \GENERICCONSULTINGCOMPANY\\
        A general firm that provides any other type of advice, such as: financial advice on the full range of strategic transactions, including mergers, sell-side and buy-side advisories, leveraged buy-outs, joint ventures, spin-offs, split-offs, divestitures, recapitalizations, exchange offers, takeover defenses, restructurings as well as shareholder relations; accountability advice; due diligence advice; etc.
        We decided to use the \GENERICCONSULTINGCOMPANY label also when it’s impossible to determine the role of the advisor based on the information reported in the document.\\
        
    \end{itemize}
    \item[(c)] \Info\\
    Set of the labels defined for identifying transaction info.\\
    \begin{itemize}
        \item \LOIDATE\\
        The date when a not definitive agreement (Letter-Of-Intent, i.e. LOI) was signed. 
        We considered only the dates occurring in contexts from which it’s linguistically clear that the date is an LOI signing date. 
        For example, we did not tag the date in the dateline, even if it’s the same as the LOI signing date.
        Moreover, we decided to include also relative dates (like ``today'' or ``yesterday''), date spans (such as ``last week'' or ``first quarter'') and incomplete dates (such as ``2020'').\\
        
        \item \ANNUALREVENUES\\
        The annual revenues of the \ACQUIREDCOMPANY, if it is present. 
        With this label, we intended to identify entities as: sales, operating revenues, net revenues, net sales, gross revenues, total revenues.\\
        
    \end{itemize}
\end{itemize}

\end{comment}

==> tables/tagset_v2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  The TAGSET Structure v2
%
\begin{comment}
\begin{table*}[ht!]\centering
    \caption{Generated by Spread-LaTeX}\label{tab: }
    \scriptsize
    \begin{tabular}{ccll}\toprule
        \textbf{Group} &\textbf{Data point} &\textbf{Description} \\\midrule
        \Parties    &                   & Groups data points used to identify the entities directly involved in the transaction. \\
                    & \ACQUIREDCOMPANY   & The company target of the transaction. \\
                    & \BUYINGCOMPANY     & The company which is acquiring the target \\
                    & \SELLINGCOMPANY    & The company which is selling the target \\
        \Advisors   &                   & Groups data points identifying any external facilitators and advisors of the transaction \\
                    & \CONSULTANT        & Individual professionals (either independent or of respective consulting firm) advising on the transactions. \\
                    & \LEGALCONSULTINGCOMPANY & A law firm providing advice on mergers and acquisitions, such as: government regulation, litigation, anti-trust, structured finance, tax etc.\\
                    & \GENERICCONSULTINGCOMPANY & A general firm that provides any other type of advice, such as: financial, accountability, due diligence, etc. \\
        \Info       &                   & Set of the labels defined for identifying transaction info. \\
                    & \ANNUALREVENUES    & The annual revenues of the \ACQUIREDCOMPANY, if it is present. \\
    \bottomrule
    \end{tabular}
\end{table*}
\end{comment}
